VLM Q-Learning: Aligning Vision-Language Models for Interactive Decision-Making

Recent research looks to harness the general knowledge and reasoning of large language models (LLMs) into agents that accomplish user-specified goals in interactive environments. Vision-language models (VLMs) extend LLMs to multi-modal data and provide agents with the visual reasoning necessary for new applications in areas such as computer automation. However, agent tasks emphasize skills where accessible open-weight VLMs lag behind their LLM equivalents. For example, VLMs are less capable of following an environment's strict output syntax requirements and are more focused on open-ended question answering. Overcoming these limitations requires supervised fine-tuning (SFT) on task-specific expert demonstrations. Our work approaches these challenges from an offline-to-online reinforcement learning (RL) perspective. RL lets us fine-tune VLMs to agent tasks while learning from the unsuccessful decisions of our own model or more capable (larger) models. We explore an off-policy RL solution that retains the stability and simplicity of the widely used SFT workflow while allowing our agent to self-improve and learn from low-quality datasets. We demonstrate this technique with two open-weight VLMs across three multi-modal agent domains.

==> tables/gym_cards_prompting.tex <==

\begin{table}[h!]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}lcccccc@{}}
\toprule
\multicolumn{1}{c}{} & \textbf{\begin{tabular}[c]{@{}c@{}}Random\\ Valid Actions\end{tabular}} & {\ul \textbf{MoonDream2}} & {\ul \textbf{PaliGemma}} & {\ul \textbf{xGen-MM}} & {\ul \textbf{Gemma2B}} & {\ul \textbf{xLAM}} \\ \midrule
NumberLine-v0        & 58 (100)                                                                & 0 (0)                     & 0 (0)                    & 53 (83)                & 0 (0)                  & 100 (100)           \\
Blackjack-v0         & 28 (100)                                                                & 0 (0)                     & 0 (0)                    & 32 (55)                & 0 (0)                  & 13 (100)            \\ \bottomrule
\end{tabular}}
\label{tbl:gym_cards_prompt_results}
\caption{test caption}
\end{table}
